Sampling Correctors

In many situations, sample data is obtained from a noisy or imperfect source. In order to address such corruptions, this paper introduces the concept of a sampling corrector. Such algorithms use structure that the distribution is purported to have, in order to allow one to make "on-the-fly" corrections to samples drawn from probability distributions. These algorithms then act as filters between the noisy data and the end user. We show connections between sampling correctors, distribution learning algorithms, and distribution property testing algorithms. We show that these connections can be utilized to expand the applicability of known distribution learning and property testing algorithms as well as to achieve improved algorithms for those tasks. As a first step, we show how to design sampling correctors using proper learning algorithms. We then focus on the question of whether algorithms for sampling correctors can be more efficient in terms of sample complexity than learning algorithms for the analogous families of distributions. When correcting monotonicity, we show that this is indeed the case when also granted query access to the cumulative distribution function. We also obtain sampling correctors for monotonicity without this stronger type of access, provided that the distribution be originally very close to monotone (namely, at a distance $O(1/\log^2 n)$). In addition to that, we consider a restricted error model that aims at capturing "missing data" corruptions. In this model, we show that distributions that are close to monotone have sampling correctors that are significantly more efficient than achievable by the learning approach. We also consider the question of whether an additional source of independent random bits is required by sampling correctors to implement the correction process.

==> preamble.tex <==
\makeatletter
\@ifundefined{theorem}{%
  % Theorems (each with its own style, all same counter). Cf. http://ftp.math.purdue.edu/mirrors/ctan.org/macros/latex/contrib/hyperref/doc/manual.pdf, p.17
  \theoremstyle{plain}
  	\newtheorem{theorem}{Theorem}[section]
  	\newaliascnt{corollary}{theorem}
  		\newtheorem{corollary}[corollary]{Corollary}
	\aliascntresetthe{corollary}
  	\newaliascnt{lemma}{theorem}
  		\newtheorem{lemma}[lemma]{Lemma}
  	\aliascntresetthe{lemma}
  	\newaliascnt{claim}{theorem}
  		\newtheorem{claim}[claim]{Claim}
	\aliascntresetthe{claim}
	\newaliascnt{fact}{theorem}
 	 	\newtheorem{fact}[fact]{Fact}
	\aliascntresetthe{fact}
  	\newtheorem*{unnumberedfact}{Fact}
  	\newaliascnt{proposition}{theorem}
  		\newtheorem{proposition}[proposition]{Proposition}
	\aliascntresetthe{proposition}
  \theoremstyle{remark}
    \newaliascnt{rk}{theorem}
  	\newtheorem{remark}[rk]{Remark}
  	\aliascntresetthe{proposition}
%   	\newtheorem{question}[theorem]{Question}
  	\newtheorem*{notation}{Notation}
%  	 \newtheorem{example}[theorem]{Example}
  \theoremstyle{definition}
  \newaliascnt{defn}{theorem}
 	 \newtheorem{definition}[defn]{Definition}
}{}
\makeatother
\providecommand*{\lemmaautorefname}{Lemma} % For \autoref{} to know the name of lemmata
\providecommand*{\claimautorefname}{Claim}
\providecommand*{\corollaryautorefname}{Corollary}
\providecommand*{\algorithmname}{Algorithm}
\providecommand*{\defnname}{Definition}
\providecommand*{\factautorefname}{Fact}
\providecommand*{\rkautorefname}{Remark}
\newenvironment{proofof}[1]{\begin{proof}[Proof of {#1}]}{\end{proof}}

%% \email{} command
\providecommand{\email}[1]{\href{mailto:#1}{\nolinkurl{#1}\xspace}}

%% Remarks and notes
\ifnum\withcolors=1
  \newcommand{\new}[1]{{\color{red} {#1}}} % New stuff
  \newcommand{\newer}[1]{{\color{RoyalPurple} {#1}}} % Newer stuff
  \newcommand{\newest}[1]{{\color{orange} {#1}}} % Even even newer stuff
  \newcommand{\newerest}[1]{{\color{ForestGreen} {#1}}} % Even even newer stuff
\else
  \newcommand{\new}[1]{{{#1}}}
  \newcommand{\newer}[1]{{{#1}}}
  \newcommand{\newest}[1]{{{#1}}}
  \newcommand{\newerest}[1]{{{#1}}}
\fi

\usepackage[colorinlistoftodos,textsize=scriptsize]{todonotes}
\ifnum\withnotes=1
  \newcommand{\rcolor}[1]{{\color{orange}#1}} % Ronitt
  \newcommand{\tcolor}[1]{{\color{green}#1}} % Themis
  \newcommand{\ccolor}[1]{{\color{RubineRed}#1}} % Clement
  \newcommand{\rnote}[1]{\par\rcolor{\textbf{R:} \sf #1}} % Ronitt
  \newcommand{\tnote}[1]{\par\tcolor{\textbf{T:} \sf #1}} % Themis
  \newcommand{\cnote}[1]{\par\ccolor{\textbf{C:} \sf #1}} % Clement
	\newcommand{\todonote}[1]{\todo[size=\scriptsize,color=red!40]{#1}}
	\newcommand{\marginnote}[1]{\todo[color=white,linecolor=black]{#1}}
\else
  \newcommand{\rcolor}[1]{{#1}}
  \newcommand{\tcolor}[1]{{#1}}
  \newcommand{\ccolor}[1]{{#1}}
  \newcommand{\rnote}[1]{{}}
  \newcommand{\tnote}[1]{{}}
  \newcommand{\cnote}[1]{{}}
  \newcommand{\todonote}[1]{\ignore{#1}}
  \newcommand{\marginnote}[1]{\ignore{#1}}
\fi
\newcommand{\rmargin}[1]{\marginnote{\rnote{#1}}}
\newcommand{\cmargin}[1]{\marginnote{\cnote{#1}}}
\newcommand{\tmargin}[1]{\marginnote{\tnote{#1}}}
\newcommand{\ignore}[1]{\leavevmode\unskip}

% Shortcuts
\newcommand{\eps}{\ensuremath{\varepsilon}\xspace}
\newcommand{\Algo}{\ensuremath{\mathcal{A}}\xspace} % Algorithm A
\newcommand{\Tester}{\ensuremath{\mathcal{T}}\xspace} % Testing algorithm T
\newcommand{\Learner}{\ensuremath{\mathcal{L}}\xspace} % Learning algorithm L
\newcommand{\property}{\ensuremath{\mathcal{P}}\xspace} % Property P
\newcommand{\class}{\ensuremath{\mathcal{C}}\xspace} % Class C
\newcommand{\eqdef}{\stackrel{\rm def}{=}}
\newcommand{\eqlaw}{\stackrel{\mathcal{L}}{=}}
\newcommand{\accept}{\textsf{ACCEPT}\xspace}
\newcommand{\fail}{\textsf{FAIL}\xspace}
\newcommand{\reject}{\textsf{REJECT}\xspace}
\newcommand{\opt}{{\textsc{opt}}\xspace}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\Domain}{\ensuremath{\Omega}\xspace} % Domain of a distribution (default notation)

% Complexity
\newcommand{\littleO}[1]{{o\!\left({#1}\right)}}
\newcommand{\bigO}[1]{{O\!\left({#1}\right)}}
\newcommand{\bigTheta}[1]{{\Theta\!\left({#1}\right)}}
\newcommand{\bigOmega}[1]{{\Omega\!\left({#1}\right)}}
\newcommand{\tildeO}[1]{\tilde{O}\!\left({#1}\right)}
\newcommand{\tildeTheta}[1]{\operatorname{\tilde{\Theta}}\!\left({#1}\right)}
\providecommand{\poly}{\operatorname*{poly}}

% Sets and indicators
\newcommand{\setOfSuchThat}[2]{ \left\{\; #1 \;\colon\; #2\; \right\} } 			% sets such as "{ elems | condition }"
\newcommand{\indicSet}[1]{\mathds{1}_{#1}}                                              % indicator function
\newcommand{\indic}[1]{\indicSet{\left\{#1\right\}}}                                             % indicator function
\newcommand{\disjunion}{\amalg}%\coprod, \dotcup...

% Distance
\newcommand{\totalvardist}[2]{{\operatorname{d_{\rm TV}}\!\left({#1, #2}\right)}}
\newcommand{\kolmogorov}[2]{{\operatorname{d_{\rm K}}\!\left({#1, #2}\right)}}

% Probability
\newcommand{\proba}{\Pr}
\newcommand{\probaOf}[1]{\proba\!\left[\, #1\, \right]}
\newcommand{\probaCond}[2]{\proba\!\left[\, #1 \;\middle\vert\; #2\, \right]}
\newcommand{\probaDistrOf}[2]{\proba_{#1}\left[\, #2\, \right]}

% Support of a distribution/function
\newcommand{\supp}[1]{\operatorname{supp}\!\left(#1\right)}

% Expectation & variance
\newcommand{\expect}[1]{\mathbb{E}\!\left[#1\right]}
\newcommand{\expectCond}[2]{\mathbb{E}\!\left[\, #1 \;\middle\vert\; #2\, \right]}
\newcommand{\shortexpect}{\mathbb{E}}
\newcommand{\var}{\operatorname{Var}}

% Distributions
\newcommand{\uniform}{\ensuremath{\mathcal{U}}}
\newcommand{\uniformOn}[1]{\ensuremath{\uniform\!\left( #1 \right) }}
\newcommand{\geom}[1]{\ensuremath{\operatorname{Geom}\!\left( #1 \right)}}
\newcommand{\bernoulli}[1]{\ensuremath{\operatorname{Bern}\!\left( #1 \right)}}
\newcommand{\binomial}[2]{\ensuremath{\operatorname{Bin}\!\left( #1, #2 \right)}}
\newcommand{\poisson}[1]{\ensuremath{\operatorname{Poisson}\!\left( #1 \right) }}
\newcommand{\gaussian}[2]{\ensuremath{ \mathcal{N}\!\left(#1,#2\right) }}
\newcommand{\gaussianpdf}[2]{\ensuremath{ g_{#1,#2}}}
\newcommand{\betadistr}[2]{\ensuremath{ \operatorname{Beta}\!\left( #1, #2 \right) }}

% Norms
\newcommand{\norm}[1]{\lVert#1{\rVert}}
\newcommand{\normone}[1]{{\norm{#1}}_1}
\newcommand{\normtwo}[1]{{\norm{#1}}_2}
\newcommand{\norminf}[1]{{\norm{#1}}_\infty}
\newcommand{\abs}[1]{\left\lvert #1 \right\rvert}
\newcommand{\dabs}[1]{\lvert #1 \rvert}

% Ceiling and floor
\newcommand{\clg}[1]{\left\lceil #1 \right\rceil}
\newcommand{\flr}[1]{\left\lfloor #1 \right\rfloor}

% Common sets
\newcommand{\R}{\ensuremath{\mathbb{R}}\xspace}
\newcommand{\C}{\ensuremath{\mathbb{C}}\xspace}
\newcommand{\Q}{\ensuremath{\mathbb{Q}}\xspace}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}\xspace}
\newcommand{\N}{\ensuremath{\mathbb{N}}\xspace}
\newcommand{\cont}[1]{\ensuremath{\mathcal{C}^{#1}}}

% Oracles and variants
\newcommand{\ICOND}{{\sf INTCOND}\xspace}
\newcommand{\EVAL}{{\sf EVAL}\xspace}
\newcommand{\CDFEVAL}{{\sf CEVAL}\xspace}
\newcommand{\STAT}{{\sf STAT}\xspace}
\newcommand{\SAMP}{{\sf SAMP}\xspace}
\newcommand{\COND}{{\sf COND}\xspace}
\newcommand{\PCOND}{{\sf PAIRCOND}\xspace}

\newcommand{\ORACLE}{{\sf ORACLE}\xspace}
\newcommand{\lp}[1][1]{\ell_{#1}}
\newcommand{\domain}{\ensuremath{\mathcal{X}}\xspace}

% Convolution
\DeclareMathOperator{\convolution}{\ast}

%% Terminology
\newcommand{\D}{\ensuremath{D}}
\newcommand{\distrD}{\ensuremath{\mathcal{D}}}
\newcommand{\birge}[2][\D]{\Phi_{#2}(#1)}
\newcommand{\iid}{i.i.d.\xspace}
\newcommand{\cdf}{cdf\xspace}
\newcommand{\pdfsamp}{dual\xspace}
\newcommand{\cdfsamp}{cumulative dual\xspace}
\newcommand{\Pdfsamp}{\expandafter\capitalisewords\expandafter{\pdfsamp}}
\newcommand{\Cdfsamp}{\expandafter\capitalisewords\expandafter{\cdfsamp}}


% Short version details
\ifnum\fulldetails=1
\newcommand{\shortversiononly}[1]{\leavevmode\unskip}
\else
\newcommand{\shortversiononly}[1]{#1}
\fi


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Add author and title info to PDF (and handles multiple authors)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
  \AtBeginDocument{
  \begingroup
  \toks@={}%
  \toksdef\toks@@=2 %
  \toks@@={}%
  \long\def\@ReturnFiFi#1#2\fi\fi{\fi\fi#1}%
  \def\scan@author#1#2 \and#3\@nil{%
  \ifx\\#3\\%
    \ifcase#1 %
      \toks@={#2}%
    \else
      \ifnum#1>1 %
        \toks@=\expandafter{%
          \the\expandafter\toks@\expandafter,\expandafter\space
          \the\toks@@
        }%
      \fi
      \toks@=\expandafter{\the\toks@\space and #2}%
    \fi
    \else
      \ifcase#1 %
        \toks@={#2}%
        \@ReturnFiFi{%
          \scan@author1#3\@nil
        }%
      \else
        \ifnum#1>1 %
          \toks@=\expandafter{%
            \the\expandafter\toks@\expandafter,\expandafter\space
            \the\toks@@
          }%
      \fi
      \toks@@={#2}%
      \@ReturnFiFi{%
        \scan@author2#3\@nil
      }%
    \fi
  \fi
  }%
  \expandafter\expandafter\expandafter\scan@author
  \expandafter\expandafter\expandafter0%
  \expandafter\@author\space\and\@nil
  \edef\x{\endgroup
  \noexpand\hypersetup{pdfauthor={\the\toks@}}%
  }%
  \x
  }
\makeatother

\makeatletter
\newcommand*{\inlineequation}[2][]{%
  \begingroup
    % Put \refstepcounter at the beginning, because
    % package `hyperref' sets the anchor here.
    \refstepcounter{equation}%
    \ifx\\#1\\%
    \else
      \label{#1}%
    \fi
    % prevent line breaks inside equation
    \relpenalty=10000 %
    \binoppenalty=10000 %
    \ensuremath{%
      % \displaystyle % larger fractions, ...
      #2%
    }%
    ~\@eqnnum
  \endgroup
}
\makeatother

%%%%%%%%%%%%%%% Hack for thm-restate
\ifnum\withthmrestate=1
	\usepackage{thm-restate}
\else
	\newenvironment{restatable}[3][]{%
		\begin{theorem}[#1]
		}{%
		\end{theorem}
	}
\fi

